Towards Races in Linear Logic

Process calculi based in logic, such as $\pi$DILL and CP, provide a foundation for deadlock-free concurrent programming, but exclude non-determinism and races. HCP is a reformulation of CP which addresses a fundamental shortcoming: the fundamental operator for parallel composition from the $\pi$-calculus does not correspond to any rule of linear logic, and therefore not to any term construct in CP. We introduce non-deterministic HCP, which extends HCP with a novel account of non-determinism. Our approach draws on bounded linear logic to provide a strongly-typed account of standard process calculus expressions of non-determinism. We show that our extension is expressive enough to capture many uses of non-determinism in untyped calculi, such as non-deterministic choice, while preserving HCP's meta-theoretic properties, including deadlock freedom.

==> fig-cp-preservation-equiv.tex <==
\begin{figure*}[htb]
  \centering
  \begin{tabular}{ll}
    \cpEquivLinkComm
    &
      \begin{prooftree*}
        \AXC{}
        \NOM{Ax}
        \UIC{$\seq[{ \cpLink{x}{y} }]{ \tmty{x}{A}, \tmty{y}{A^\bot} }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{}
        \NOM{Ax}
        \UIC{$\seq[{ \cpLink{y}{x} }]{ \tmty{y}{A^\bot}, \tmty{x}{A^{\bot\bot}} }$}
        \RightLabel{$(\cdot)^\bot$-Involutive}
        \UIC{$\seq[{ \cpLink{y}{x} }]{ \tmty{y}{A^\bot}, \tmty{x}{A} }$}
      \end{prooftree*}
    \\[25pt]
    \cpEquivCutComm
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A^\bot} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{P}{Q} }]{ \Gamma, \Delta }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A^\bot} }$}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A} }$}
        \RightLabel{$(\cdot)^\bot$-Involutive}
        \UIC{$\seq[{ P }]{ \Gamma, \tmty{x}{A^{\bot\bot}} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{Q}{P} }]{ \Gamma, \Delta }$}
      \end{prooftree*}
    \\[25pt]
    \cpEquivCutAss1
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A^\bot}, \tmty{y}{B} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{y}{B^\bot} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{y}{Q}{R} }]{ \Delta, \Theta, \tmty{x}{A^\bot} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{P}{\cpCut{y}{Q}{R}} }]{ \Gamma, \Delta, \Theta }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A^\bot}, \tmty{y}{B} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{P}{Q} }]{ \Gamma, \Delta, \tmty{y}{B} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{y}{B^\bot} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{y}{\cpCut{x}{P}{Q}}{R} }]{ \Gamma, \Delta, \Theta }$}
      \end{prooftree*}
  \end{tabular}
  \caption{Type preservation for the structural congruence of \cp}
  \label{fig:cp-preservation-equiv}
\end{figure*}
%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> fig-cp-preservation.tex <==
\begin{figure*}[htb]
  \begin{tabular}{ll}
    \cpRedAxCut1
    &
      \begin{prooftree*}
        \AXC{}
        \NOM{Ax}
        \UIC{$\seq[{ \cpLink{w}{x} }]{ \tmty{w}{A}, \tmty{x}{A^\bot} }$}
        \AXC{$\seq[{ R }]{ \tmty{x}{A}, \Gamma }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{\cpLink{w}{x}}{R} }]{ \tmty{w}{A}, \Gamma }$}
      \end{prooftree*}
    \\[20pt]
    $\Longrightarrow$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ \cpSub{w}{x}{R} }]{ \tmty{w}{A}, \Gamma }$}
      \end{prooftree*}
    \\[20pt]
    
    \cpRedBetaTensParr
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A^\bot}, \tmty{y}{B^\bot} }$}
        \SYM{\parr}
        \UIC{$\seq[{ \cpRecv{y}{x}P }]{ \Gamma, \tmty{y}{A^\bot \parr B^\bot} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{y}{B} }$}
        \SYM{\tens}
        \BIC{$\seq[{ \cpSend{y}{x}(Q \mid R) }]{ \Delta, \Theta, \tmty{y}{A \tens B} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{y}{\cpRecv{y}{x}{P}}{\cpSend{y}{x}{Q}{R}} }]{ \Gamma, \Delta, \Theta }$}
      \end{prooftree*}
    \\[20pt]
    $\Longrightarrow$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A^\bot}, \tmty{y}{B^\bot} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{P}{Q} }]{ \Gamma, \Delta, \tmty{y}{B^\bot} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{y}{B} }$}      
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{y}{\cpCut{x}{P}{Q}}{R} }]{ \Gamma, \Delta, \Theta }$}
      \end{prooftree*}
    \\[25pt]
    
    \cpRedBetaOneBot
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma }$}
        \SYM{\bot}
        \UIC{$\seq[{ \cpWait{x}{P} }]{ \Gamma, \tmty{x}{\bot} }$}
        \AXC{}
        \SYM{\one}
        \UIC{$\seq[{ \cpHalt{x} }]{ \tmty{x}{\one} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{\cpHalt{x}}{\cpWait{x}{P}} }]{ \Gamma }$}
      \end{prooftree*}
    \\[20pt]
    $\Longrightarrow$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma }$}
      \end{prooftree*}
    \\[25pt]
    
    \cpRedBetaPlusWith1
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A^\bot} }$}
        \AXC{$\seq[{ Q }]{ \Gamma, \tmty{x}{B^\bot} }$}
        \SYM{\with}
        \BIC{$\seq[{ \cpCase{x}{P}{Q} }]{ \Gamma, \tmty{x}{A^\bot \with B^\bot} }$}
        \AXC{$\seq[{ R }]{ \Delta, \tmty{x}{A} }$}
        \SYM{\plus_1}
        \UIC{$\seq[{ \cpInl{x}{R}}]{ \Delta, \tmty{x}{A \plus B} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{\cpCase{x}{P}{Q}}{\cpInl{x}{R}} }]{ \Gamma, \Delta }$}
      \end{prooftree*}
    \\[20pt]
    $\Longrightarrow$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{A^\bot} }$}
        \AXC{$\seq[{ R }]{ \Delta, \tmty{x}{A} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{P}{R} }]{ \Gamma, \Delta }$} 
      \end{prooftree*}
    \\[25pt]
    
    \cpRedBetaPlusWith2
    &
      (as above)
  \end{tabular}
  
  \caption{Type preservation for the \cpRedAxCut1 and \textbeta-reduction rules of \cp}
  \label{fig:cp-preservation}
\end{figure*}
%%% Local Variables:
%%% TeX-master: "main"
%%% End:

==> fig-nc-local-choice.tex <==
\begin{sidewaysfigure}[ht]
  \begin{landscape}
    \begin{prooftree}
      \AXC{}
      \SYM{(\one)}
      \UIC{$\seq[{ \cpHalt{y} }]{ \tmty{y}{\one} }$}
      \SYM{(\plus_1)}
      \UIC{$\seq[{ \cpInl{y}{\cpHalt{y}} }]{ \tmty{y}{\one \plus \one} }$}
      \SYM{(\take[1]{})}
      \UIC{$\seq[{ \ncCnt{x}{y}{\cpInr{y}{\cpHalt{y}}} }]{ \tmty{x}{\take[1]{\one \plus \one}} }$}
      
      \AXC{}
      \SYM{(\one)}
      \UIC{$\seq[{ \cpHalt{z} }]{ \tmty{z}{\one} }$}
      \SYM{(\plus_2)}
      \UIC{$\seq[{ \cpInr{z}{\cpHalt{z}} }]{ \tmty{z}{\one \plus \one} }$}
      \SYM{(\take[1]{})}
      \UIC{$\seq[{ \ncCnt{x}{z}{\cpInr{z}{\cpHalt{z}}} }]{ \tmty{x}{\take[1]{\one \plus \one}} }$}
      
      \NOM{Pool}
      \BIC{$\seq[{
          \ncPool{\ncCnt{x}{y}{\cpInr{y}{\cpHalt{y}}}}{\ncCnt{x}{y}{\cpInr{y}{\cpHalt{y}}}}
        }]{
          \tmty{x}{\take[2]{\one \plus \one}}
        }$}
    \end{prooftree}
    \vspace*{1\baselineskip}
    \begin{prooftree}
      \AXC{$\seq[{ P }]{ \Gamma }$}
      \SYM{(\bot)} 
      \UIC{$\seq[{ \cpWait{z}{P} }]{ \Gamma, \tmty{z}{\bot} }$}
      \AXC{$\seq[{ P }]{ \Gamma }$}
      \SYM{(\bot)} 
      \UIC{$\seq[{ \cpWait{z}{P} }]{ \Gamma, \tmty{z}{\bot} }$}
      \SYM{(\with)}
      \BIC{$\seq[{ \cpCase{z}{\cpWait{z}{P}}{\cpWait{z}{P}} }]{
          \Gamma, \tmty{z}{\bot\with\bot} }$}
      \SYM{(\bot)} 
      \UIC{$\seq[{ \cpWait{z}{\cpCase{z}{\cpWait{z}{P}}{\cpWait{z}{P}}} }]{
          \Gamma, \tmty{z}{\bot\with\bot}, \tmty{y}{\bot} }$}
 
      \AXC{$\seq[{ Q }]{ \Gamma }$}
      \SYM{(\bot)} 
      \UIC{$\seq[{ \cpWait{z}{Q} }]{ \Gamma, \tmty{z}{\bot} }$}
      \AXC{$\seq[{ Q }]{ \Gamma }$}
      \SYM{(\bot)} 
      \UIC{$\seq[{ \cpWait{z}{Q} }]{ \Gamma, \tmty{z}{\bot} }$}
      \SYM{(\with)}
      \BIC{$\seq[{ \cpCase{z}{\cpWait{z}{Q}}{\cpWait{z}{Q}} }]{
          \Gamma, \tmty{z}{\bot\with\bot} }$}
      \SYM{(\bot)} 
      \UIC{$\seq[{ \cpWait{z}{\cpCase{z}{\cpWait{z}{Q}}{\cpWait{z}{Q}}} }]{
          \Gamma, \tmty{z}{\bot\with\bot}, \tmty{y}{\bot} }$}
      
      \SYM{(\with)}
      \BIC{$\seq[{
          \cpCase{y}{\cpWait{y}{\cpCase{z}{\cpWait{z}{P}}{\cpWait{z}{P}}}}{\cpWait{y}{\cpCase{z}{\cpWait{z}{Q}}{\cpWait{z}{Q}}}}
        }]{ \Gamma, \tmty{z}{\bot\with\bot}, \tmty{y}{\bot\with\bot} }$} 
      \SYM{(\give[1]{})}
      \UIC{$\seq[{
          \ncSrv{x'}{z}{\cpCase{y}{\cpWait{y}{\cpCase{z}{\cpWait{z}{P}}{\cpWait{z}{P}}}}{\cpWait{y}{\cpCase{z}{\cpWait{z}{Q}}{\cpWait{z}{Q}}}}}
        }]{ \Gamma, \tmty{x'}{\give[1]{\bot\with\bot}}, \tmty{y}{\bot\with\bot} }$}
      \SYM{(\give[1]{})}
      \UIC{$\seq[{
          \ncSrv{x}{y}{\ncSrv{x'}{z}{\cpCase{y}{\cpWait{y}{\cpCase{z}{\cpWait{z}{P}}{\cpWait{z}{P}}}}{\cpWait{y}{\cpCase{z}{\cpWait{z}{Q}}{\cpWait{z}{Q}}}}}}
        }]{ \Gamma, \tmty{x'}{\give[1]{\bot\with\bot}}, \tmty{x}{\give[1]{\bot\with\bot}} }$} 
      \NOM{Cont}
      \UIC{$\seq[{
          \ncSrv{x}{y}{\ncSrv{x}{z}{\cpCase{y}{\cpWait{y}{\cpCase{z}{\cpWait{z}{P}}{\cpWait{z}{P}}}}{\cpWait{y}{\cpCase{z}{\cpWait{z}{Q}}{\cpWait{z}{Q}}}}}}
        }]{ \Gamma, \tmty{x}{\give[1]{\bot\with\bot}}, \tmty{x}{\give[1]{\bot\with\bot}} }$} 
    \end{prooftree}
  \end{landscape}
  \caption{Derivations for the encoding of non-deterministic local choice in \nodcap.}
  \label{fig:nc-local-choice}
\end{sidewaysfigure}
%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> fig-nc-preservation-equiv.tex <==
\begin{figure*}[h!tb]
  \centering
  \begin{tabular}{ll}
    \ncEquivPoolComm
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{\take[m]{A}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[n]{A}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{Q} }]{ \Gamma, \Delta, \take[m+n]{A} }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[n]{A}} }$}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{\take[m]{A}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{Q}{P} }]{ \Gamma, \Delta, \tmty{x}{\take[m+n]{A}} }$}
      \end{prooftree*}
    \\[25pt]
    \ncEquivPoolAss1
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{\take[l]{A}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[m]{A}} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{x}{\take[n]{A}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{Q}{R} }]{ \Delta, \Theta, \tmty{x}{\take[m+n]{A}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{\ncPool{Q}{R}} }]{ \Gamma, \Delta, \Theta, \tmty{x}{\take[l+m+n]{A}} }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{\take[l]{A}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[m]{A}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{Q} }]{ \Gamma, \Delta, \tmty{x}{\take[l+m]{A}} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{x}{\take[n]{A}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{\ncPool{P}{Q}}{R} }]{ \Gamma, \Delta, \Theta, \tmty{x}{\take[l+m+n]{A}} }$}
      \end{prooftree*}
    \\[5pt]
    or
    \\[5pt]
    \ncEquivPoolAss1
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{\take[k]{A}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[l]{A}}, \tmty{y}{\take[m]{B}} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{y}{\take[n]{B}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{Q}{R} }]{ \Delta, \Theta, \tmty{x}{\take[l]{A}}, \tmty{y}{\take[m+n]{B}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{\ncPool{Q}{R}} }]{ \Gamma, \Delta, \Theta, \tmty{x}{\take[k+l]{A}}, \tmty{y}{\take[m+n]{B}} }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{x}{\take[k]{A}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[l]{A}}, \tmty{y}{\take[m]{B}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{Q} }]{ \Gamma, \Delta, \tmty{x}{\take[k+l]{A}}, \tmty{y}{\take[m]{B}} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{x}{\take[n]{B}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{\ncPool{P}{Q}}{R} }]{ \Gamma, \Delta, \Theta, \tmty{x}{\take[k+l]{A}}, \tmty{y}{\take[m+n]{B}} }$}
      \end{prooftree*}
    \\[20pt]
    \ncRedKappaPool1
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{y}{\take[m]{B}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A}, \tmty{y}{\take[n]{B}} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{x}{A^\bot} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{Q}{R} }]{ \Gamma, \Delta, \Theta, \tmty{y}{\take[n]{B}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{\cpCut{x}{Q}{R}} }]{ \Gamma, \Delta, \Theta, \tmty{y}{\take[m+n]{B}} }$}
      \end{prooftree*}
    \\[20pt]
    $\equiv$
    &
      \begin{prooftree*}
        \AXC{$\seq[{ P }]{ \Gamma, \tmty{y}{\take[m]{B}} }$}
        \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{A}, \tmty{y}{\take[n]{B}} }$}
        \NOM{Pool}
        \BIC{$\seq[{ \ncPool{P}{Q} }]{ \Gamma, \Delta, \tmty{x}{A}, \tmty{y}{\take[m+n]{B}} }$}
        \AXC{$\seq[{ R }]{ \Theta, \tmty{x}{A^\bot} }$}
        \NOM{Cut}
        \BIC{$\seq[{ \cpCut{x}{\ncPool{P}{Q}}{R} }]{ \Gamma, \Delta, \Theta, \tmty{y}{\take[m+n]{B}} }$}
      \end{prooftree*} 
    \\[20pt]
    \ncRedKappaPool2
    &
      (as above)
  \end{tabular}
  \caption{Type preservation for the structural congruence of \nodcap}
  \label{fig:nc-preservation-equiv}
\end{figure*}
%%% Local Variables:
%%% TeX-master: "main"
%%% End:


==> fig-nc-preservation.tex <==
\begin{figure*}[htb]
  \makebox[\textwidth][c]{
    \begin{tabular}{ll}
      \ncRedBetaStar1
      &
        \begin{prooftree*}
          \AXC{$\seq[{ P }]{ \Gamma, \tmty{y}{A} }$}
          \SYM{\take[1]{}}
          \UIC{$\seq[{ \ncCnt{x}{y}{P} }]{ \Gamma, \tmty{x}{\take[1]{A}} }$}
          \AXC{$\seq[{ Q }]{ \Delta, \tmty{z}{A^\bot} }$}
          \SYM{\give[1]{}}
          \UIC{$\seq[{ \ncSrv{x}{z}{Q} }]{ \Delta, \tmty{x}{\give[1]{A^\bot}} }$}
          \NOM{Cut}
          \BIC{$\seq[{ \cpCut{x}{\ncCnt{x}{y}{P}}{\ncSrv{x}{z}{Q}} }]{ \Gamma, \Delta }$}
        \end{prooftree*}
      \\[20pt]
      $\Longrightarrow$
      &
        \begin{prooftree*}
          \AXC{$\seq[{ P }]{ \Gamma, \tmty{y}{A} }$}
          \AXC{$\seq[{ Q }]{ \Delta, \tmty{z}{A^\bot} }$}
          \NOM{Cut}
          \BIC{$\seq[{ \cpCut{y}{P}{\cpSub{y}{z}{Q}} }]{ \Gamma, \Delta }$}
        \end{prooftree*}
      \\[25pt]
      \ncRedBetaStar{n+1}
      &
        \begin{prooftree*}
          \AXC{$\seq[{ P }]{ \Gamma, \tmty{y}{A} }$}
          \SYM{\take[1]{}}
          \UIC{$\seq[{ \ncCnt{x}{y}{P} }]{ \Gamma, \tmty{x}{\take[1]{A}} }$}
          \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[n]{A}} }$}
          \NOM{Pool}
          \BIC{$\seq[{ \ncPool{\ncCnt{x}{y}{P}}{Q} }]{ \Gamma, \Delta, \tmty{x}{\take[n+1]{A}} }$}
          \AXC{$\seq[{ R }]{ \Theta, \tmty{z}{A^\bot}, \tmty{x}{\give[n]{A^\bot}} }$}
          \SYM{\give[1]{}}
          \UIC{$\seq[{ \ncSrv{x'}{z}{Q} }]{ \Theta, \tmty{x'}{\give[1]{A^\bot}}, \tmty{x}{\give[n]{A^\bot}} }$}
          \NOM{Cont}
          \UIC{$\seq[{ \ncSrv{x}{z}{Q} }]{ \Theta, \tmty{x}{\give[n+1]{A^\bot}} }$}
          \NOM{Cut}
          \BIC{$\seq[{ \cpCut{x}{\ncPool{\ncCnt{x}{y}{P}}{Q}}{\ncSrv{x}{z}{Q}} }]{ \Gamma, \Delta, \Theta }$}
        \end{prooftree*}
      \\[25pt]
      $\Longrightarrow$
      &
        \begin{prooftree*}
          \AXC{$\seq[{ Q }]{ \Delta, \tmty{x}{\take[n]{A}} }$}
          \AXC{$\seq[{ P }]{ \Gamma, \tmty{y}{A} }$}
          \AXC{$\seq[{ R }]{ \Theta, \tmty{z}{A^\bot}, \tmty{x}{\give[n]{A}} }$}
          \NOM{Cut}
          \BIC{$\seq[{ \cpCut{y}{P}{\cpSub{y}{z}{R}} }]{ \Gamma, \Theta, \tmty{x}{\give[n]{A}} }$}
          \NOM{Cut}
          \BIC{$\seq[{ \cpCut{x}{Q}{\cpCut{y}{P}{\cpSub{y}{z}{R}}} }]{ \Gamma, \Delta, \Theta }$}
        \end{prooftree*}
    \end{tabular}
  }   

  \caption{Type preservation for the \textbeta-reduction rules of \nodcap}
  \label{fig:nc-preservation}
\end{figure*}
%%% Local Variables:
%%% TeX-master: "main"
%%% End: 
